Requirements Development for IoT Systems with UCM4IoT

The engineering of IoT (Internet of Things) systems brings about various challenges due to the inherent complexities associated with such adaptive systems. Addressing the adaptive nature of IoT systems in the early stages of the development life cycle is essential for developing a complete and precise system specification. In this paper, we propose a use case-based modelling language, UCM4IoT, to support requirements elicitation and specification of IoT systems. UCM4IoT takes into account the heterogeneity of IoT systems and provides domain-specific language constructs to model the different facets of IoT systems. The language also incorporates the notion of exceptional situations and adaptive system behaviour. Our language is supported with a textual modelling environment to assist modellers in writing use cases. The environment supports syntax-directed editing, validation of use case models, and requirements analysis. The proposed language and tool is demonstrated and evaluated with two case studies: smart store system and smart fire alarm system.

==> analysis.tex <==
%\section{Analysis}
%\label{sec:tooling}

%\emph{Tabassum - TO DO: Check if the text in this section is still valid.}

%\textcolor{red}{Tabassum- Add the handler summary table analysis}

%UCM4IoT enables modellers to perform analysis on the generated exception summary tables
%UCM4IoT enables modellers to perform path-based analysis on the generated exception summary tables.

%In this way, it is possible to determine how critical a handler is to the system's success by analyzing the number of possible sequences that depend on the success of that handler. 
%Similarly, it is also possible to determine how important it is to handle an exception based on the number of sequences it appears.

% Could talk about actors and their importance, but don't have enough examples on single actors vs. multiple actors.


